Contextual Bandit with Adaptive Feature Extraction

We consider an online decision making setting known as contextual bandit problem, and propose an approach for improving contextual bandit performance by using an adaptive feature extraction (representation learning) based on online clustering. Our approach starts with an off-line pre-training on unlabeled history of contexts (which can be exploited by our approach, but not by the standard contextual bandit), followed by an online selection and adaptation of encoders. Specifically, given an input sample (context), the proposed approach selects the most appropriate encoding function to extract a feature vector which becomes an input for a contextual bandit, and updates both the bandit and the encoding function based on the context and on the feedback (reward). Our experiments on a variety of datasets, and both in stationary and non-stationary environments of several kinds demonstrate clear advantages of the proposed adaptive representation learning over the standard contextual bandit based on "raw" input contexts.

==> sec_IJCAI_head.tex <==

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}

\def\Rset{\mathbb{R}}
%\def\C{\mathbb{C}}
\def\N{\mathbb{N}}
\def\Z{\mathbb{Z}}
\def\E{\mathbb{E}}
\def\P{\mathbb{P}}
\def\T{\mathcal{T}}
\def\Var{\mathbb{V}ar}
\def\rme{\operatorname{e}}
\newcommand{\1}[1]{\mathbbm{1}_{\left\{#1\right\}}}
\DeclareMathOperator*{\argmax}{arg\,max}

\def\ps{P}\def\Ps{\P_\pi}\def\mus{\mu}\def\Es{\E_\pi}
\def\Xb{\bar{X}}
\def\F{\mathcal{F}}\def\A{\mathcal{A}}
\def\eqdef{\triangleq}

% \captionsetup[subfigure]{labelformat=simple,labelsep=colon}
% \renewcommand{\thesubfigure}{fig\arabic{subfigure}}

% Following comment is from ijcai97-submit.tex:
% The preparation of these files was supported by Schlumberger Palo Alto
% Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
% Shirley Jowell, of Morgan Kaufmann Publishers, and Peter F.
% Patel-Schneider, of AT\&T Bell Laboratories collaborated on their
% preparation.

% These instructions can be modified and used in other conferences as long
% as credit to the authors and supporting agencies is retained, this notice
% is not changed, and further modification or reuse is not restricted.
% Neither Shirley Jowell nor Peter F. Patel-Schneider can be listed as
% contacts for providing assistance without their prior permission.

% To use for other conferences, change references to files and the
% conference appropriate and use other authors, contacts, publishers, and
% organizations.
% Also change the deadline and address for returning papers and the length and
% page charge instructions.
% Put where the files are available in the appropriate places.

==> sec_acknowledgement.tex <==
\subsection*{Acknowledgments}

==> sec_backup_tables.tex <==
\begin{table}[tbh]
	\centering
	\caption{Non-stationary Environment with  with Unshuffled Reward Function (till t = 8000)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l  | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST & \textbf{37.24} & 34.44 & 29.00 & 22.32 \\
			STL-10 &  10.29 & \textbf{15.81} & 14.77 & 13.43 \\
			CIFAR-10 & 9.62 & \textbf{14.30} & 13.30 & 11.73 \\
			Caltech-101 S & \textbf{1.18} & 1.14 & 1.09 & 1.06 \\
            Warfarin & \textbf{62.58} & 56.7 & 56.1 & 56.92 \\
			\hline
            mix: MNIST/Warfarin & 44.29 & 50.43 \textbf{53.23} & 48.94 \\
            \hline
		\end{tabular}
	}  
\label{table:nonstatAccUnshuffled8000}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Non-stationary Environment with  with Shuffled Reward Function (till t = 8000)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l  | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST & 12.19 & \textbf{33.75} & 29.04 & 23.83 \\
			STL-10 &  10.05 & \textbf{16.64} & 15.10 & 12.77 \\
			CIFAR-10 & 10.23 & \textbf{14.83} & 13.13 & 11.60 \\
			Caltech-101 S & 1.00 & 1.09 & 1.23 & \textbf{1.30} \\
            Warfarin & 40.66 & \textbf{55.10} & 50.56 & 54.44 \\
			\hline
            mix: MNIST/Warfarin & 23.54 & 49.33 & \textbf{50.67} & 49.15 \\
            \hline
		\end{tabular}
	}  
\label{table:nonstatAccShuffled8000}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Non-stationary Environment with  with Unshuffled Reward Function (till end)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l  | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST & \textbf{37.24} & 34.44 & 29.00 & 22.32 \\
			STL-10 &  10.29 & \textbf{15.81} & 14.77 & 13.43 \\
			CIFAR-10 & 9.62 & \textbf{14.30} & 13.30 & 11.73 \\
			Caltech-101 S & \textbf{1.18} & 1.14 & 1.09 & 1.06 \\
            Warfarin & \textbf{62.58} & 56.7 & 56.1 & 56.92 \\
			\hline
            mix: MNIST/Warfarin & 45.76 & 50.58 & \textbf{51.21} & 47.74\\
            \hline
		\end{tabular}
	}  
\label{table:nonstatAccUnshuffled}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Non-stationary Environment with  with Shuffled Reward Function (till end)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l  | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST & 12.19 & \textbf{33.75} & 29.04 & 23.83 \\
			STL-10 &  10.05 & \textbf{16.64} & 15.10 & 12.77 \\
			CIFAR-10 & 10.23 & \textbf{14.83} & 13.13 & 11.60 \\
			Caltech-101 S & 1.00 & 1.09 & 1.23 & \textbf{1.30} \\
            Warfarin & 40.66 & \textbf{55.10} & 50.56 & 54.44 \\
			\hline
            mix: MNIST/Warfarin & 23.54 & 49.33 & \textbf{50.67} & 49.15 \\
            \hline
		\end{tabular}
	}  
\label{table:nonstatAccShuffled}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Negative Environment with Unshuffled Reward Function (till t = 8000)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST half-stat & 10.21 & 14.06 & 14.26 & \textbf{16.46} \\
			MNIST rand-stat & 10.49 & 17.06 & 16.00 & \textbf{21.54} \\
			MNIST half-nonStat & 10.48 & 25.06 & \textbf{25.16} & 23.99 \\
			MNIST rand-nonStat & 10.30 & 24.04 & 28.43 & \textbf{28.50}  \\  \hline
            STL-10 half-stat & 10.13 & 10.49 & \textbf{10.50} & 10.21 \\
            STL-10 rand-stat &  9.68 & \textbf{12.45} & 12.25 & 10.29 \\
            STL-10 half-nonStat & 9.55 & 11.25 & \textbf{12.25} & 11.63 \\
            STL-10 rand-nonStat & 9.90 & 13.00 & \textbf{14.30} & 11.60 \\
			\hline
            Caltech-101 S half-stat &  0.98 & \textbf{10.04} & 7.98 & 6.94 \\
            Caltech-101 S rand-stat & 0.94 & 10.93 & 8.40 & \textbf{11.68}  \\
            Caltech-101 S half-nonStat & 1.04 & 1.20 & \textbf{1.23} & 0.96 \\
            Caltech-101 S rand-nonStat & 0.96 & 1.09 & \textbf{1.20} & 0.99 \\
			\hline
		\end{tabular}
	}
	\label{table:AccUnshuffledNeg8000}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Negative Environment with Shuffled Reward Function (till t = 8000)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST half-stat & 9.94 & 14.43 & 14.25 & \textbf{16.63} \\
			MNIST rand-stat & 9.80 & \textbf{18.83} & 16.50 & 17.83  \\
			MNIST half-nonStat & 9.86 & 21.51 & \textbf{26.99} & 24.84 \\
			MNIST rand-nonStat & 9.85 & 24.59 & 24.96 & \textbf{31.69} \\ \hline
            STL-10 half-stat & 9.48 & \textbf{11.90} 10.64 & 10.48 \\
            STL-10 rand-stat & 10.04 & 11.46 & \textbf{12.48} & 11.39  \\
            STL-10 half-nonStat & 10.35 & 11.81 & \textbf{13.44} & 11.01  \\
            STL-10 rand-nonStat & 9.25 & \textbf{12.03} & 11.88 & 11.71  \\
			\hline
            Caltech-101 S half-stat &  1.11 & \textbf{8.71} & 6.21 & 7.93 \\
            Caltech-101 S rand-stat & 0.94 & \textbf{10.36} & 9.11 & 3.38 \\
            Caltech-101 S half-nonStat & 1.06 & 1.03 & 1.00 & \textbf{1.29} \\
            Caltech-101 S rand-nonStat & 1.08 & 1.05 & 1.13 & \textbf{1.16} \\
			\hline
		\end{tabular}
	}
	\label{table:AccShuffledNeg8000}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Negative Environment with Unshuffled Reward Function (till end)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST half-stat & 13.50 & 14.70 & 14.02 & \textbf{16.18} \\
			MNIST rand-stat & 13.72 & 17.14 & 15.53 & \textbf{17.70}  \\
			MNIST half-nonStat & 14.45 & 25.09 & 23.82 & \textbf{26.90} \\
			MNIST rand-nonStat & 14.05 & 24.38 & 25.90 & \textbf{28.43}   \\  \hline
            STL-10 half-stat & 10.06 & \textbf{10.42} & 10.33 & 10.04 \\
            STL-10 rand-stat & 9.77 & \textbf{12.34} & 12.33 & 10.41 \\
            STL-10 half-nonStat & 9.88 & 10.99 & \textbf{12.29} & 11.56 \\
            STL-10 rand-nonStat & 9.85 & 12.99 & \textbf{13.67} & 11.55 \\
			\hline
            Caltech-101 S half-stat &  0.98 & \textbf{10.04} & 7.98 & 6.94 \\
            Caltech-101 S rand-stat & 0.94 & 10.93 & 8.40 & \textbf{11.68}  \\
            Caltech-101 S half-nonStat & 1.04 & 1.20 & \textbf{1.23} & 0.96 \\
            Caltech-101 S rand-nonStat & 0.96 & 1.09 & \textbf{1.20} & 0.99 \\
			\hline
		\end{tabular}
	}
	\label{table:AccUnshuffledNeg}
\end{table}

\begin{table}[tbh]
	\centering
	\caption{Negative Environment with Shuffled Reward Function (till end)}
	\resizebox{0.92\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l }
			Datasets & baseline & uE & mE &  oE  \\ \hline 
			MNIST half-stat & 10.22  & 14.59 & 13.86 & \textbf{14.79} \\
			MNIST rand-stat & 9.87 & \textbf{17.84} & 14.35 & 17.32  \\
			MNIST half-nonStat & 10.78 & 23.02 & 22.33 & \textbf{26.84} \\
			MNIST rand-nonStat & 11.27 & 27.34 & 24.87 & \textbf{28.36} \\ \hline
            STL-10 half-stat & 9.66 & \textbf{11.51} & 10.73 & 10.60 \\
            STL-10 rand-stat & 9.95 & 11.44 & \textbf{12.37} & 11.17 \\
            STL-10 half-nonStat & 10.31 & 11.86 & \textbf{13.17} & 11.19  \\
            STL-10 rand-nonStat & 9.2 & \textbf{12.62} & 12.49 & 11.59  \\
			\hline
            Caltech-101 S half-stat &  1.11 & \textbf{8.71} & 6.21 & 7.93 \\
            Caltech-101 S rand-stat & 0.94 & \textbf{10.36} & 9.11 & 3.38 \\
            Caltech-101 S half-nonStat & 1.06 & 1.03 & 1.00 & \textbf{1.29} \\
            Caltech-101 S rand-nonStat & 1.08 & 1.05 & 1.13 & \textbf{1.16} \\
			\hline
		\end{tabular}
	}
	\label{table:AccShuffledNeg}
\end{table}


% \begin{table*}[tbh]
% 	\centering
% 	\caption{Non-stationary Environment in short term (till t = 8000)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l }%| l }
% 			Datasets & baseline & mini-batch embedding &  on-line embedding  & mini-batch-history CB & full-history CB \\ \hline % & mini-batch context \\ \hline
% % 			Datasets \\ \hline % & \multicolumn{5}{c|}{on-line learning setting} & mini-batch setting \\ \hline
% 			MNIST & $ 14.85 $ & $\textbf{29.42} \pm \textbf{1.17}$ & $23.95\pm 2.15$ & $20.40\pm 6.68$ & $23.02\pm 6.66$ \\% & $32.38 \pm 0.59$\\
% 			STL-10 &  $10.23 $ & $\textbf{14.05} \pm \textbf{0.96}$ & $12.11 \pm 1.28$ & $11.87 \pm 1.42$	& $12.45\pm 1.32$ \\% & $14.08 \pm 0.57$\\
% 			CIFAR-10 & $9.39$ & $\textbf{12.84} \pm \textbf{0.59}$ & $11.16\pm0.62$ & $11.38 \pm 0.67$ & $11.30 \pm 1.16$ \\% & $12.95 \pm 0.51$\\
% 			Caltech-101 S & $\textbf{1.18}$ & $ 1.04 \pm 0.07$ & $1.02\pm 0.04$ & $1.05\pm 0.08$ & $1.09\pm 0.08$* \\% & $1.06 \pm 0.27$\\
% 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:nonstatAcc}
% \end{table*}
 
% \begin{table*}[tbh]
% 	\centering
% 	\caption{Non-stationary Environment with  with Unshuffled Reward Function (till end)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l | l | l }%| l }
% 			Datasets & baseline & uE & mE &  oE  & mhCB & fhCB & mmhCB & mmfhCB \\ \hline % & mini-batch context \\ \hline
% % 			Datasets \\ \hline % & \multicolumn{5}{c|}{on-line learning setting} & mini-batch setting \\ \hline
% 			MNIST & \textbf{37.24} & 34.45  & 27.53 $\pm$ 2.02 & 19.76 $\pm$ 2.55 & 18.95 $\pm$ 3.44 & 21.35 $\pm$ 5.65 & 15.24 $\pm$ 2.14 & 18.12 $\pm$ 1.79 \\
% 			STL-10 & 10.29 & \textbf{15.81} & 14.11 $\pm$ 0.66 & 12.15 $\pm$ 1.11 & 11.60 $\pm$ 1.39 & 12.42 $\pm$ 1.30 & 11.38 $\pm$ 0.25 & 11.70 $\pm$ 0.75 \\
% 			CIFAR-10 & 9.62 & \textbf{14.30} & 12.94 $\pm$ 0.46 & 11.36 $\pm$ 0.51 & 11.26 $\pm$ 0.45 & 11.32 $\pm$ 1.11 & 10.49 $\pm$ 0.34 & 10.40 $\pm$ 0.65 \\
% 			Caltech-101 S & \textbf{1.18} & 1.14 & 1.04 $\pm$ 0.07 & 1.02 $\pm$ 0.04 & 1.05 $\pm$ 0.08 & 1.09 $\pm$ 0.08 & 0.97 $\pm$ 0.12 & 1.09 $\pm$ 0.08 \\
%             Warfarin & \textbf{62.58} & 56.70 & 53.77 $\pm$ 2.89 & 52.94 $\pm$ 3.58 & 53.38 $\pm$ 3.89 & 54.40 $\pm$ 2.14 & 51.21 $\pm$ 1.50 & 54.31 $\pm$ 3.61 \\
% 			\hline
%             mix: MNIST/Warfarin &  45.76  & &  \textbf{49.99} $\pm$ \textbf{1.78} & 44.92 $\pm$ 2.46 & 36.04 $\pm$ 7.55 & 45.39 $\pm$ 5.87 & 29.77 $\pm$ 4.49 & 38.25 $\pm$ 2.64 \\
%             mix: MNIST/STL-10 & \\
%             \hline
% 		\end{tabular}
% 	}
% 	\label{table:nonstatAccUnshuffled}
% \end{table*}

% \begin{table*}[tbh]
% 	\centering
% 	\caption{Non-stationary Environment with Shuffled Reward Function (till end)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l | l | l }%| l }
% 			Datasets & baseline & uE & mE &  oE  & mhCB & fhCB & mmhCB & mmfhCB \\ \hline % & mini-batch context \\ \hline
% % 			Datasets \\ \hline % & \multicolumn{5}{c|}{on-line learning setting} & mini-batch setting \\ \hline
% 			MNIST & 12.19 & \textbf{33.75} & 26.85 $\pm$ 2.62 & 19.10 $\pm$ 4.46 & 19.23 $\pm$ 5.00 & 20.45 $\pm$ 4.64 & 15.31 $\pm$ 2.31 & 16.09 $\pm$ 3.30 \\
% 			STL-10 & 10.05 & \textbf{16.64} & 14.20  $\pm$ 1.21 & 12.24 $\pm$ 0.64 & 12.00 $\pm$ 1.93 & 12.18 $\pm$ 1.26 & 11.24 $\pm$ 0.11 & 11.04 $\pm$ 0.59 \\
% 			CIFAR-10 & 10.23 & \textbf{14.83} & 12.74 $\pm$ 0.46 & 11.15 $\pm$ 0.39 & 11.37 $\pm$ 1.17 & 11.62 $\pm$ 1.13 & 10.54 $\pm$ 0.62 & 10.72 $\pm$ 0.37 \\
% 			Caltech-101 S & 1.00  &  1.09 & \textbf{1.16} $\pm$ \textbf{0.06} & 1.12 $\pm$ 0.16 & 1.07 $\pm$ 0.19 & 1.02 $\pm$ 0.19 & 1.12 $\pm$ 0.05 & 1.10 $\pm$ 0.03 \\
%             Warfarin & 40.66 & \textbf{55.10} & 48.61 $\pm$ 3.25 & 51.38 $\pm$ 3.01 & 50.30 $\pm$ 3.03 & 51.41 $\pm$ 5.29 & 49.14 $\pm$ 3.67 & 49.19 $\pm$ 3.69 \\
%             \hline
%             mix: MNIST/Warfarin & 23.54  & \textbf{49.33} & 49.00 $\pm$ 1.45 & 42.67 $\pm$ 5.99 & 35.23 $\pm$ 7.70 & 40.61 $\pm$ 6.66 & 28.88 $\pm$ 5.22 & 38.35 $\pm$ 5.15 \\
%             mix: MNIST/STL-10 \\
% 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:nonstatAccShuffled}
% \end{table*}



% \begin{table*}[tbh]
% 	\centering
% 	\caption{Negative Environment with Unshuffled Reward Function (till end)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l | l | l }%| l }
% 			Datasets & baseline & uE & mE &  oE  & mhCB & fhCB & mmhCB & mmfhCB \\ \hline % & mini-batch context \\ \hline
% % 			Datasets \\ \hline % & \multicolumn{5}{c|}{on-line learning setting} & mini-batch setting \\ \hline
% 			MNIST half-stat & 13.50 & 14.70 & 14.02 & \textbf{16.18} & 10.93 & 13.74 & 10.22 & 11.12 \\
% 			MNIST rand-stat & 13.72 & 17.14 & 15.53 & \textbf{17.70} & 11.99 & 13.87 & 10.77 & 12.00 \\
% 			MNIST half-nonStat & 14.44 & 25.09 & 23.82 &  \textbf{26.90} & 17.41 & 22.28 & 12.58 & 15.62  \\
% 			MNIST rand-nonStat & 14.05 & 24.38 & 25.90 & \textbf{28.43} & 20.43 & 24.26 & 15.61 & 17.23 \\  \hline
%             STL-10 half-stat & 10.06 & 10.42 & 10.33 & 10.04 & 10.39 & 10.22 & \textbf{10.46} & 10.21 \\
%             STL-10 rand-stat & 9.77 & \textbf{12.34} & 12.33* & 10.41 & 11.26 & 11.41 & 10.96 & 11.15 \\
%             STL-10 half-nonStat & 9.88 & 10.99 & 12.29 & \textbf{11.56} & 11.47 & 11.15 & 10.65 & 9.96 \\
%             STL-10 rand-nonStat & 9.85 & 12.99 & \textbf{13.67} & 11.55 & 11.78 & 11.77 & 10.36 & 10.21 \\
% 			\hline
%             Caltech-101 S half-stat & 0.98 & \textbf{10.04 }& 7.98 & 6.94 & 4.46 & 6.06 & 1.69 & 1.88 \\
%             Caltech-101 S rand-stat & 0.94 & 10.93 & 8.40 & \textbf{11.68} & 10.40 & 6.26 & 1.70 & 3.81 \\
%             Caltech-101 S half-nonStat & 1.0375 & 1.20 & 1.23 & 0.96 & \textbf{1.36} & 1.13 & 1.04 & 1.00 \\
%             Caltech-101 S rand-nonStat & 0.96 & 1.09 & \textbf{1.20} & 0.99 & 0.99 & 0.93 & 1.19* & 1.09 \\
% 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:AccUnshuffledNeg}
% \end{table*}

% \begin{table*}[tbh]
% 	\centering
% 	\caption{Negative Environment with Shuffled Reward Function (till end)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l | l | l }%| l }
% 			Datasets & baseline & uE & mE &  oE  & mhCB & fhCB & mmhCB & mmfhCB \\ \hline % & mini-batch context \\ \hline
% % 			Datasets \\ \hline % & \multicolumn{5}{c|}{on-line learning setting} & mini-batch setting \\ \hline
% 			MNIST half-stat & 10.22 & 14.59 & 13.86 & \textbf{14.79} & 11.26 & 12.84 & 10.62 & 10.78 \\
% 			MNIST rand-stat & 9.87 & \textbf{17.84} & 14.35 & 17.32 & 11.91 & 15.12 & 10.94 & 11.74 \\
% 			MNIST half-nonStat & 10.78 & 23.02 & 22.33 & \textbf{26.84} & 18.48 & 21.87 & 13.28 & 15.28 \\
% 			MNIST rand-nonStat & 11.27 & 27.34 & 24.87 & \textbf{28.36} & 19.05 & 22.81 & 14.63 & 17.22 \\ \hline
%             STL-10 half-stat & 9.66 & \textbf{11.51} & 10.73 & 10.60 & 10.34 & 10.96 & 11.00 & 10.01 \\
%             STL-10 rand-stat & 9.95 & 11.44 & \textbf{12.37} & 11.17 & 11.52 & 11.59 & 10.21 & 10.59 \\
%             STL-10 half-nonStat & 10.31 & 11.86 & \textbf{13.17} & 11.19 & 10.94 & 10.85 & 10.37 & 10.74 \\
%             STL-10 rand-nonStat & 9.20 & \textbf{12.62} & 12.49 & 11.59 & 11.89 & 11.04 & 10.42 & 10.68 \\
% 			\hline
%             Caltech-101 S half-stat & 1.11 & \textbf{8.71} & 6.21 & 7.93 & 4.33 & 6.15 & 1.75 & 1.84 \\
%             Caltech-101 S rand-stat & 0.94 & \textbf{10.36} & 9.11 & 3.38 & 6.40 & 7.66 & 1.75 & 4.84 \\
%             Caltech-101 S half-nonStat & 1.06 & 1.03 & 1.00 & 1.29 & 1.10 & 1.25 & 1.08 & \textbf{1.36} \\
%             Caltech-101 S rand-nonStat & 1.08 & 1.05 & 1.13 & 1.16 & \textbf{1.33} & 1.13 & 1.04 & 1.31 \\
% 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:AccShuffledNeg}
% \end{table*}

% \begin{table*}[tbh]
% 	\centering
% 	\caption{Adaptive Compression with Budgeted Selection Reward ($\alpha_k = 0.5$, $\alpha_p = 0$)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l }
% 			Datasets & 100\% & 50\% & 25\% & 5\% & mini-batch-history CB &  full-history CB \\ \hline % 
% 			Warfarin - unshuffled - linear & \textbf{62.32} & 61.14 & 60.86 & 60.26 & 59.76 (avg. comp. = 52.18\%) & 58.94 (avg. comp. = 34.17\%) \\
%             Warfarin - unshuffled - autoencoder & \textbf{57.98} & 57.64 & 56.74 & 47.58 & 55.82 (avg. comp. = 45.47\%) & 57.44 (avg. comp. = 49.64\%) \\
%             Warfarin - shuffled - linear & 40.48 & 43.76 & 38.92 & 46.70 & \textbf{52.28} (avg. comp. = 44.25) & 51.36 (avg. comp. = 47.41\%) \\
%             Warfarin - shuffled - autoencoder & \textbf{57.06} & 55.58 & 53.94 & 39.50 & 52.28 (avg. comp. = 44.25) & 51.36 (avg. comp. = 47.41\%)\\
%             \hline
% % 			MNIST - unshuffled - linear & \\
% %             MNIST - unshuffled - autoencoder & \\
% % 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:alpha_0.5_0}
% \end{table*}

% \begin{table*}[tbh]
% 	\centering
% 	\caption{Adaptive Compression with Budgeted Final Reward ($\alpha_k = 0.5$, $\alpha_p = 0.5$)}
% 	\resizebox{1.84\columnwidth}{!}{
% 		\begin{tabular}{ l | l | l | l | l | l | l }
% 			Datasets & 100\% & 50\% & 25\% & 5\% & mhCB & fhCB \\ \hline % 
% 			Warfarin - unshuffled - linear &  \textbf{62.06} & 61.10 & 60.56 & 59.20 & 59.96 (avg. comp. = 36.59\%) &  59.16 (avg. comp. = 38.21\%)\\
%             Warfarin - unshuffled - autoencoder & 56.94 & 55.98 & 54.82 & 53.02 & 54.20 (avg. comp. = 46.87\%) & \textbf{57.44} (avg. comp. = 49.64\%)\\
%             Warfarin - shuffled - linear & 40.48 & \textbf{43.76} & 38.92 & 40.68 & 41.10 (avg. comp. = 49.14 \%) & 42.04 (avg. comp. = 39.42\%)\\
%             Warfarin - shuffled - autoencoder & \textbf{57.06} & 55.58 & 53.94 & 39.50 & 52.64 (avg. comp. = 46.94\%) & 50.86 (avg. comp. = 44.32\%)\\
%             \hline
% % 			MNIST - unshuffled - linear & \\
% %             MNIST - unshuffled - autoencoder & \\
% % 			\hline
% 		\end{tabular}
% 	}
% 	\label{table:alpha_0.5_0.5}
% \end{table*}

==> sec_compression.tex <==
\subsection{Adaptive Compression with Context-Dependent Embeddings}

\begin{algorithm}%[H]
	\caption{\small Adaptive Compression with Context-Dependent Embeddings}
	\label{alg:compression}
	\begin{algorithmic}[1]
   \STATE {\bfseries } \textbf{Input:}  $\textbf{D}$, a set of unlabeled contexts (data for pre-training); $\textbf{k}$, a series of available compression levels (embeddings); a Boolean condition defining a specific method from algorithmic family: $isStagedCB$.
   \STATE {\bfseries } \textbf{Initialization:} 
\STATE {\bfseries} \quad for each compression level within vector \textbf{k}, construct a set of encoding functions (embeddings): \textbf{E} = {$e_1, ..., e_k$} 
 \STATE {\bfseries} \quad initialize contextual Thompson Sampling parameters for compression level selection bandit $B_1$ and classification-decision bandit $B_2$.
   \STATE {\bfseries } \textbf{While} there is a next data mini-batch $M_l$, \textbf{do}
   \STATE {\bfseries } \quad  \textbf{Foreach} $x_i$ from mini-batch $M_l$ \textbf{do}
    \STATE {\bfseries }    \quad\quad    $e = selectCompressionCB(B_1,x_i$)\\
    \STATE {\bfseries }    \quad\quad  $z = e(x_i)$
    \STATE {\bfseries }    \quad\quad  $d = contextualBandit(B_2,z$)
       \STATE {\bfseries }    \quad\quad Receive reward $r_i(d)$ 
       \STATE  {\bfseries }    \quad\quad $[r_i^k, r_i^p] = assignReward(\alpha_k, \alpha_p, r_i(d))$ 
    \STATE {\bfseries }    \quad \quad $updateBandit(r_i^k, B_1)$\\
    \STATE {\bfseries }    \quad \quad $updateBandit(r_i^p, B_2)$\\
     \quad \textbf{End}
    \STATE {\bfseries }   \quad$updateEmbedding(M_l,\textbf{k}$)
     \STATE {\bfseries }   \quad \textbf{If} $isStagedCB$  \textbf{then}   $reinitializeCB$ \\
\textbf{End}
   \end{algorithmic}
\end{algorithm}

To explore the application of the algorithm in adaptive compression, here we describe an algorithmic scheme (Algorithm \ref{alg:compression}) which extended \textit{mini-batch-history CB (mhCB)} and \textit{full-history CB (mhCB)} with embeddings defined as different compression level. The two bandits, compression level selection bandit $B_1$ and classification-decision bandit $B_2$, each were given their own budgeted reward with function $assignReward$, defined as $r^k = r - \alpha_k * c$ and $r^p = r - \alpha_p * c$ where $c$ is the compression level, with $100\%$ meaning full conservation of all information. During training, we defined embeddings in two different approaches: a linear compression and an autoencoder trained with $n$ nodes in the hidden layer where $n = c*D$ ($D$ is the input dimension).



